Optically identified BL Lacertae objects from the Sloan Digital Sky Survey

We present a sample of 386 BL Lacertae (BL Lac) candidates identified from 2860 deg^2 of the Sloan Digital Sky Survey (SDSS) spectroscopic database. The candidates are primarily selected to have quasi-featureless optical spectra and low proper motions as measured from SDSS and USNO-B positions; however, our ability to separate Galactic from extragalactic quasi-featureless objects (QFOs) on the basis of proper motion alone is limited by the lack of reliable proper motion measurements for faint objects. Fortunately, high proper motion QFOs, mostly DC white dwarfs, populate a well defined region of color space, approximately corresponding to blackbodies with temperatures in the range 7000-12000 K. QFOs with measurable redshifts or X-ray or radio counterparts (i.e., evidence of an extragalactic/AGN nature) loosely follow a track in color space that corresponds to power-law continua plus host galaxy starlight, with typical power-law slopes in the range 1<alpha_{opt}<2 (f_{nu} propto nu^{-alpha}). Based largely on this remarkably clean color separation, we subdivide the sample into 240 probable candidates and 146 additional less probable (likely stellar) candidates. The probable BL Lac candidates have multi-wavelength properties consistent with the range of previously known BL Lacs, with an apparent preponderance of objects with synchrotron peaks at relatively high energies (HBL/ XBL-type). The majority of the 154 objects with measurable redshifts have z<1, with a median of 0.45; there are also a handful of high-redshift objects extending up to z=5.03. We identify a small number of potential radio-quiet BL Lac candidates, although more sensitive radio observations are needed to confirm their radio-quiet nature.

==> tab1_short.tex <==
\startdata
 SDSS J012227.38$+$151023.1  &  20.34$\pm$0.05  &  19.90$\pm$0.02  &  19.55$\pm$0.03  &  19.25$\pm$0.03  &  18.93$\pm$0.05  &  0.17  &  p  &    1048580  &         \nodata  &    7.1  &        N  \\ 
 SDSS J012716.31$-$082128.9  &  20.26$\pm$0.07  &  19.70$\pm$0.03  &  19.14$\pm$0.03  &  18.81$\pm$0.02  &  18.55$\pm$0.04  &  0.08  &  p  &         20  &          0.362?  &    4.1  &        Y  \\ 
 SDSS J012750.83$-$001346.6  &  21.03$\pm$0.09  &  20.66$\pm$0.04  &  19.83$\pm$0.02  &  19.30$\pm$0.03  &  18.95$\pm$0.04  &  0.09  &  r  &    2097154  &          0.4376  &    6.0  &        N  \\ 
 SDSS J013408.95$+$003102.5  &  21.17$\pm$0.10  &  20.22$\pm$0.03  &  19.90$\pm$0.02  &  19.72$\pm$0.03  &  19.79$\pm$0.08  &  0.07  &  p  &          2  &         \nodata  &  154.5?  &        N  \\ 
 SDSS J014125.83$-$092843.7  &  18.11$\pm$0.02  &  17.59$\pm$0.03  &  17.21$\pm$0.02  &  16.96$\pm$0.01  &  16.68$\pm$0.02  &  0.08  &  p  &       7700  &     $\geq 0.5$?  &    5.8  &        Y  \\ 
 SDSS J020106.18$+$003400.2  &  18.90$\pm$0.02  &  18.62$\pm$0.02  &  18.25$\pm$0.03  &  17.99$\pm$0.02  &  17.80$\pm$0.02  &  0.07  &  r  &       5636  &          0.2985  &    7.6  &        Y  \\ 
 SDSS J020137.66$+$002535.1*  &  20.39$\pm$0.05  &  20.06$\pm$0.02  &  19.54$\pm$0.02  &  19.39$\pm$0.02  &  19.38$\pm$0.09  &  0.08  &  p  &    1048576  &         \nodata  &  176.1?  &        N  \\ 
 SDSS J022048.46$-$084250.4  &  18.92$\pm$0.02  &  18.62$\pm$0.03  &  18.27$\pm$0.02  &  18.03$\pm$0.02  &  17.80$\pm$0.03  &  0.06  &  p  &    1056276  &         0.5252?  &    7.1  &        N  \\ 
 SDSS J023813.68$-$092431.4  &  20.86$\pm$0.09  &  20.27$\pm$0.03  &  19.63$\pm$0.02  &  19.22$\pm$0.03  &  18.85$\pm$0.05  &  0.08  &  r  &    2102788  &          0.4188  &    3.6  &        Y  \\ 
 SDSS J024156.38$+$004351.6  &  20.66$\pm$0.08  &  20.03$\pm$0.02  &  19.61$\pm$0.02  &  19.41$\pm$0.03  &  19.29$\pm$0.05  &  0.09  &  p  &          3  &            0.99  &    6.1?  &        N  \\ 
\enddata


==> tab2_short.tex <==
\startdata
 SDSS J012227.38$+$151023.1  &    4.29  &  U  &  \nodata  &        $<$0.03  &   178.2  &  $<$5.7  &  $<$25.7  &  \nodata  &     \nodata  &  \nodata  &      0.8  &           38.0$\pm$1.2  &  $>$0.90  &     0.50  \\ 
 SDSS J012716.31$-$082128.9  &    3.97  &  U  &  \nodata  &        $<$0.01  &   438.8  &  $<$3.2  &  $<$14.4  &     0.30  &       172.2  &     0.20  &      0.8  &          111.9$\pm$3.4  &  $>$1.04  &     0.60  \\ 
 SDSS J012750.83$-$001346.6  &    3.23  &  U  &  \nodata  &        $<$0.01  &   432.2  &  $<$2.8  &  $<$12.3  &     0.30  &         5.6  &     0.15  &      4.2  &            7.3$\pm$0.5  &  $>$0.96  &     0.38  \\ 
 SDSS J013408.95$+$003102.5  &    2.91  &  U  &  \nodata  &        $<$0.02  &   373.9  &  $<$2.6  &  $<$11.3  &  \nodata  &      $<$1.1  &     0.17  &  \nodata  &                \nodata  &  $>$0.96  &  $<$0.25  \\ 
 SDSS J014125.83$-$092843.7  &    2.66  &  F  &  19.5  &  0.03$\pm$0.01  &   440.0  &     1.5  &      6.3  &     0.20  &       517.8  &     0.15  &      0.7  &         656.7$\pm$19.7  &     1.45  &     0.54  \\ 
 SDSS J020106.18$+$003400.2  &    2.67  &  B  &   1.9  &  0.34$\pm$0.03  &   400.0  &    17.0  &     72.1  &     0.40  &        13.9  &     0.14  &      2.0  &           12.7$\pm$0.6  &     0.90  &     0.34  \\ 
 SDSS J020137.66$+$002535.1  &    2.64  &  U  &  \nodata  &        $<$0.01  &   401.4  &  $<$2.5  &  $<$10.5  &  \nodata  &      $<$1.0  &     0.15  &  \nodata  &                \nodata  &  $>$1.02  &  $<$0.22  \\ 
 SDSS J022048.46$-$084250.4  &    3.05  &  B  &   9.5  &  0.09$\pm$0.02  &   315.0  &     4.9  &     21.2  &     0.20  &        57.3  &     0.13  &      0.9  &           64.9$\pm$2.4  &     1.10  &     0.45  \\ 
 SDSS J023813.68$-$092431.4  &    2.93  &  F  &  15.3  &  0.03$\pm$0.01  &   224.0  &     1.6  &      6.8  &     0.60  &         3.0  &     0.15  &  \nodata  &                \nodata  &     1.08  &     0.31  \\ 
 SDSS J024156.38$+$004351.6  &    3.45  &  U  &  \nodata  &        $<$0.03  &   226.6  &  $<$3.9  &  $<$17.1  &  \nodata  &      $<$1.0  &     0.14  &  \nodata  &                \nodata  &  $>$0.94  &  $<$0.22  \\ 
\enddata


==> tab3_short.tex <==
\startdata
 SDSS J015604.20$-$010029.0  &  19.27$\pm$0.03  &  18.76$\pm$0.03  &  18.58$\pm$0.02  &  18.54$\pm$0.02  &  18.65$\pm$0.03  &  0.08  &  p  &          4  &   95.3?  \\ 
 SDSS J020145.70$+$011013.0  &  20.97$\pm$0.28  &  20.14$\pm$0.04  &  19.99$\pm$0.03  &  19.97$\pm$0.04  &  20.12$\pm$0.10  &  0.07  &  r  &          2  &  \nodata  \\ 
 SDSS J020712.37$+$002443.2  &  20.28$\pm$0.06  &  20.15$\pm$0.03  &  20.23$\pm$0.03  &  20.37$\pm$0.04  &  20.51$\pm$0.16  &  0.08  &  p  &    1048576  &   37.3?  \\ 
 SDSS J021142.81$+$010446.3  &  18.46$\pm$0.02  &  18.83$\pm$0.02  &  19.35$\pm$0.02  &  19.72$\pm$0.03  &  19.89$\pm$0.09  &  0.08  &  p  &    9568256  &    0.0  \\ 
 SDSS J021925.07$+$004520.3  &  20.27$\pm$0.05  &  20.17$\pm$0.03  &  20.26$\pm$0.03  &  20.29$\pm$0.04  &  20.45$\pm$0.12  &  0.10  &  p  &    1048576  &    6.4?  \\ 
 SDSS J031303.31$-$061600.5  &  20.25$\pm$0.05  &  20.23$\pm$0.02  &  20.31$\pm$0.03  &  20.41$\pm$0.05  &  20.23$\pm$0.18  &  0.16  &  p  &   34603008  &    8.6?  \\ 
 SDSS J031729.73$-$071644.7  &  20.20$\pm$0.05  &  20.01$\pm$0.03  &  20.09$\pm$0.03  &  20.29$\pm$0.04  &  20.76$\pm$0.25  &  0.15  &  p  &  537919488  &  \nodata  \\ 
 SDSS J033444.87$-$011253.9  &  20.01$\pm$0.05  &  19.95$\pm$0.03  &  19.98$\pm$0.02  &  20.20$\pm$0.03  &  20.41$\pm$0.12  &  0.40  &  p  &    1048576  &   36.2?  \\ 
 SDSS J033556.39$-$002425.5*  &  20.73$\pm$0.07  &  20.31$\pm$0.02  &  20.11$\pm$0.02  &  20.03$\pm$0.03  &  19.97$\pm$0.12  &  0.34  &  p  &          2  &   19.0?  \\ 
 SDSS J034306.18$-$054806.3  &  18.48$\pm$0.02  &  18.36$\pm$0.01  &  18.48$\pm$0.01  &  18.63$\pm$0.02  &  18.83$\pm$0.04  &  0.14  &  p  &  538443776  &   13.6?  \\ 
\enddata


==> tab4_short.tex <==
\startdata
 SDSS J015604.20$-$010029.0  &    2.57  &        $<$0.01  &   415.7  &  $<$2.4  &  $<$10.3  &      $<$1.0  &     0.14  &  $>$1.17  &  $<$0.15  \\ 
 SDSS J020145.70$+$011013.0  &    2.81  &        $<$0.01  &   410.2  &  $<$2.6  &  $<$11.0  &      $<$0.9  &     0.14  &  $>$0.95  &  $<$0.25  \\ 
 SDSS J020712.37$+$002443.2  &    2.74  &        $<$0.02  &   384.9  &  $<$2.5  &  $<$10.8  &      $<$1.0  &     0.15  &  $>$0.92  &  $<$0.27  \\ 
 SDSS J021142.81$+$010446.3  &    3.10  &        $<$0.02  &   303.5  &  $<$2.8  &  $<$11.9  &      $<$1.0  &     0.15  &  $>$1.04  &  $<$0.21  \\ 
 SDSS J021925.07$+$004520.3  &    3.17  &        $<$0.04  &   147.4  &  $<$5.7  &  $<$24.8  &      $<$0.9  &     0.13  &  $>$0.79  &  $<$0.27  \\ 
 SDSS J031303.31$-$061600.5  &    5.33  &        $<$0.03  &   226.6  &  $<$5.0  &  $<$23.5  &     \nodata  &  \nodata  &  $>$0.81  &  \nodata  \\ 
 SDSS J031729.73$-$071644.7  &    5.16  &        $<$0.02  &   271.6  &  $<$4.1  &  $<$19.2  &     \nodata  &  \nodata  &  $>$0.87  &  \nodata  \\ 
 SDSS J033444.87$-$011253.9  &    7.51  &        $<$0.01  &   536.7  &  $<$4.5  &  $<$21.9  &     \nodata  &  \nodata  &  $>$0.91  &  \nodata  \\ 
 SDSS J033556.39$-$002425.5  &    8.00  &        $<$0.01  &   526.8  &  $<$4.7  &  $<$22.7  &     \nodata  &  \nodata  &  $>$0.88  &  \nodata  \\ 
 SDSS J034306.18$-$054806.3  &    5.36  &        $<$0.01  &   409.1  &  $<$3.8  &  $<$17.9  &     \nodata  &  \nodata  &  $>$1.12  &  \nodata  \\ 
\enddata

